The Voevodsky motive of a rank one semiabelian variety

Over a perfect field k, let G be an extension of an abelian variety by the multiplicative group $\G_m$. We compute the motive of G in Voevodsky's category of etale motivic complexes with rational coefficients. The result is a decomposition similar to the classical decomposition of the Chow motive of an abelian variety obtained by Deninger/Murre, Kuennemann, Shermenev and Scholl, and other authors.

==> introduction_NF.tex <==
\begin{chapter}{Introduction}

Let $k$ be a perfect field and let $G$ be a semiabelian variety over $k$. In this thesis we study the motive $M(G)$ of $G$, in Voevodsky's category $\DMeetkQ$, of {\etl} motivic complexes with rational coefficients. Our main result (Theorem \ref{mainresult}) is that if the torus part $T$ of $G$ is $\Gm$, then there exists an isomorphism: 
\begin{align}
M(G) \simeq \Sym(\Mof(G)) := \bos_{n \ge 0} \Symn(\Mof(G)). \label{mainisom}
\end{align}
Our proof shows merely that such an isomorphism exists, without exhibiting one concretely. The proof of the isomorphy (\ref{mainisom}) relies, in an essential way, on the analogous classical decomposition:
\begin{align*}
h(A) \simeq \bos_{i \ge 0} h^{i}(A) \simeq \bos_{i \ge 0} \Sym \left( h^{1}(A) \right) 
\end{align*}
of an abelian variety $A$ in the category of effective Chow motives. Versions of this decomposition have been published by several authors: Deninger and Murre \cite{DeMu}, K{\"u}nnemann \cite{Ku1} and \cite{Ku2}, Scholl \cite{Scholl} and Shermenev \cite{Sh1}.\\\\
Let us briefly explain the notation in (\ref{mainisom}). Morally, the symmetric powers $\Symn(X)$ on $\DMeetkQ$ are $\Symn$-invariant subobjects of $X^{\ox n}$; the precise definition, taken from Biglari's work \cite[\S 2.5]{Big}, is a formal construction with idempotents that works in any $\Q$-linear pseudoabelian tensor category. The symbol $\Mof(G)$ denotes the ordinary {\etl} sheaf $\wtG := \Mor_{\Schk}(\pul{X}, G)$, regarded as a complex concentrated in degree zero. By the result \cite[Lemma 3.2]{SS} of Spie{\ss} and Szamuely, $\wtG$ has transfers and so $\Mof(G)$ is an object in $\DMeetkQ$.\\\\ 
To prove the existence of an isomorphism (\ref{mainisom}), we construct, for an arbitrary semiabelian variety $G$, a candidate morphism: 
\begin{align*}
\vp_{G}: M(G) \lra \Sym(\Mof(G)).
\end{align*}
Sadly, we are unable to show that $\vp_{G}$ is an isomorphism for a general semiabelian variety $G$ of rank $r$, or even for a general semiabelian variety of rank one; we merely use $\vp_{G}$ to prove that there must exist an isomorphism of the form (\ref{mainisom}). However, we are able to show that $\vp_{G}$ is an isomorphism in the following special cases: 
\begin{itemize}
\item[\tn{(i)}] if $G$ is an abelian variety $A$ (Proposition \ref{vpAisom}) or 
\item[\tn{(ii)}] if $G$ is a torus $T$ (Proposition \ref{vptorusisom}). 
\end{itemize} 
Moreover, we will see that $\vp_{G}$ is functorial in $G$, and multiplicative in the sense that there is a commutative diagram:
\begin{align*} 
\xymatrix@C=40pt{   
M(G \x H) \ar@{->}[dd]_(0.5){\simeqcan} \ar@{->}[rr]^(0.45){\vp_{G \x H}} & & 
 \Sym(\Mof(G \x H)) \ar@{->}[dd]^(0.5){\simeqcan} \\
& & \\
M(G) \ox M(H) \ar@{->}[rr]_(0.4){\vp_{G} \ox \vp_{H}} & & \Sym(\Mof(G)) \ox \Sym(\Mof(H)),} 
\end{align*} 
where the vertical arrows are canonical isomorphisms. From this multiplicativity and the isomorphy of $\vp_{A}$ and $\vp_{T}$, it follows that $\vp_{G}$ is also an isomorphism: 
\begin{itemize}
\item[\tn{(iii)}] if $G$ is the trivial extension $A \x T$ of $A$ by $T$ (Proposition \ref{trivextcase}). 
\end{itemize}
We also prove, in Theorem \ref{mainresult}, the following conditional result. 
\begin{itemize}
\item[\tn{(iv)}] The morphism $\vp_{G}$ is an isomorphism for any semiabelian variety $G$, provided that a certain diagram: 
\begin{align*} 
\xymatrix@C=14pt{   
M(H)(1)[2] \ar@{->}[dd]_(0.5){\vp_{H}(1)[2]} \ar@{->}[rr]^(0.52){\pd_{\Aff(G), H} \circ M(s_{0})} & & 
M(G)[1] \ar@{->}[dd]^(0.5){\vp_{G}[1]} \\
& & \\
\Sym(\Mof(H))(1)[2] \ar@{->}[rr]_(0.53){-f^{\bl}[1]} & & \Sym(\Mof(G))[1]} 
\end{align*} 
is commutative. The meaning of the symbol $H$ and the significance of the commutativity of this diagram is explained in the synopsis to Chapter 5 (see below). 
\end{itemize}
We now give a brief synopsis of this thesis, as a complement to the comprehensive introductions at the beginning of each of Chapter.\\\\
\tbf{Chapter 1.} We recall the constructions of the categories $\Chowek$ and $\DMeetkQ$, of effective Chow motives and Voevodsky motivic complexes with $\Q$ coefficients, respectively, and discuss the relationship between them. These categories are idempotent complete and have a tensor structure, which allows us to define symmetric powers $\Symn$, following Biglari \cite[\S 2.5]{Big}. The symmetric powers on $\Chowek$, $\DMegk \sx \Q$ and $\DMeetkQ$ are compatible in the sense that there are tensor functors:
\begin{align*}
& \Psi: \Chowek \lra \DMegk \sx \Q \qaq \\
& \Phi: \Chowek \lra \DMeetkQ
\end{align*}
commuting with $\Symn$ for all non-negative integers $n$.\\\\
\tbf{Chapter 2.} We construct a morphism:
\begin{align*}
\vp_{G}: M(G) \lra \Sym(\Mof(G))
\end{align*}
in the category $\DMeetkQ$ of triangulated motives, attached to a semiabelian variety $G$ over a perfect field $k$. It is functorial in $G$ and compatible with products of group schemes.\\\\
\tbf{Chapter 3.} We review the definitions of the {\SeAV} $\AXz$ and Albanese scheme $\AlbXk$ of $X$. The purpose of this is twofold. Firstly, we wish to understand the {\SeAV} because the proof in Chapter 4 that $\vp_{A}: M(A) \ra \Sym(\Mof(A))$ is an isomorphism for any abelian variety $A$ proceeds by reducing to the case where $A$ is the {\SeAV} of a smooth proper curve $C$. Secondly, understanding the Albanese scheme of $\Gm$ will allow us to prove that $\vp_{\Gm}$ is an isomorphism, implying that $\vp_{T}$ is an isomorphism for all tori $T$.\\\\
\tbf{Chapter 4.} We show that for an abelian variety $A$ over a perfect field $k$, the morphism $\vp_{A}: M(A) \ra \Sym(\Mof(A))$ is an isomorphism. The proof relies on the classical decomposition $\psi_{A}: h(A) \ira \Sym(\ho(A))$ of the motive $h(A)$ of an abelian variety in the category $\Chowek$, shown for example in \cite[Theorem 3.3.1]{Ku1}.\\\\
\tbf{Chapter 5.} We establish the existence of an isomorphism (\ref{mainisom}). The proof proceeds, firstly, by observing that any semiabelian $G$ variety of rank $r$ can be considered as an extension of an abelian variety $H$ of rank $r-1$ by $\Gm$. Thus we have a short exact sequence:
\begin{align*}
1 \lra \Gm \slra{f} G \slra{g} H \lra 0,
\end{align*}
which is used to construct the two exact triangles in $\DMeetkQ$ that form the top and bottom rows of the diagram: 
\begin{align*} 
\xymatrix@C=14pt{   
M(G) \ar@{->}[rr]^(0.5){M(g)} \ar@{->}[dd]_(0.5){\vp_{G}} & & 
M(H) \ar@{->}[rr]^(0.45){1_{M(H)} \ost c_{1}(\Aff(G))} \ar@{->}[dd]^(0.5){\vp_{H}} & & 
M(H)(1)[2] \ar@{->}[dd]^(0.5){\vp_{H}(1)[2]} \ar@{->}[rr]^(0.52){\pd_{\Aff(G), H} \circ M(s_{0})} & & 
M(G)[1] \ar@{->}[dd]^(0.5){\vp_{G}[1]} \\
& & & & & & \\
\Sym(\Mof(G)) \ar@{->}[rr]_(0.49){g^{\bl}} & & 
\Sym(\Mof(H)) \ar@{->}[rr]_(0.43){h^{\bl}} & & 
\Sym(\Mof(H))(1)[2] \ar@{->}[rr]_(0.53){-f^{\bl}[1]} & & \Sym(\Mof(G))[1],} 
\end{align*} 
We will see that the left-hand and middle squares commute, but we are unable to show that the right hand square commutes. If it did, we could use the fact that the rank of $H$ is one lower than the rank of $G$ to prove, using induction, that $\vp_{G}$ is an isomorphism. Indeed, in the base case where $r$ is zero, then $G$ is an abelian variety, and so $\vp_{G}$ is an isomorphism by Chapter 4. The inductive step then follows from a basic property of triangulated categories, namely that given any diagram depicting a morphism of triangles in which two of the vertical maps are isomorphisms, then the third map is also an isomorphism. In our case, isomorphy of $\vp_{H}$, hence also $\vp_{H}(1)[2]$, would imply that $\vp_{G}$ is an isomorphism. Even if we do not know that the right-hand square commutes, we can still conclude, by a triangulated category axiom, that there exists an isomorphism $M(G) \simeq \Sym(\Mof(G))$.

\newpage

\thispagestyle{empty}

\begin{center}
% TeX Gyre Pagella
{\fontspec{Linux Libertine O} \scshape \Large Acknowledgements}
\end{center}

{\fontspec[SizeFeatures={{Size=11.5}}]{Baskerville} I owe a great deal to my advisor, Annette Huber-Klawitter, without whose patience, support and liberally shared mathematical insights, the thesis would never have come to be. Quite apart from her formidable subject knowledge, it is impossible for me to imagine someone more dedicated to the supervision process, or more adept at steering me in the right direction. 

It is a pleasure also to thank Matthias Wendt, so generous with his time, who became a defacto coadvisor in the later stages of this work. He has a knack for explaining complex concepts in a simple way that I find inspiring, and his close reading and thoughtful comments of several drafts have made this thesis much, much better than it would have been otherwise. 

At a conference in Regensburg, Bruno Kahn not only pointed out a serious error in my work, but was kind enough to suggest an alternative strategy, which I adopted, and I thank him very warmly. 

For prompt and elucidating answers to emails containing mathematical questions, I wish to express my gratitude again to Bruno Kahn, and also to Joseph Ayoub and Klaus K{\"u}nnemann. 

For interesting mathematical and non-mathematical conversations, I am indebted to my former officemates Jakob Scholbach and Steve Meagher. I am also thankful to all my fellow doctoral students, who provided a friendly environment in which to work, and exhibited great patience with my German in seminar talks. 

This project was finanically supported by a research grant from the DFG (Research Group 570), and by teaching positions offered to me by the Mathematics Department of the Albert-Ludwigs-Universit{\"a}t Freiburg. I am very grateful to both organisations for their generosity. 

My housemates Michael Beister, Lena Dei{\ss}ler and Eva Kn{\"u}ppel make up a tremendous WG, and it's been a pleasure to live with them. For their friendship, good times and enriching conversations during my time in Freiburg, I wish to thank: Miriam Almstadt, Kalle Bues, Yue Che, Sophia Drysdale, Peer Fechner, France Foster-Thorpe, Alice Girelli, Samia Khatun, Alex K{\"onig}, Carolin Hahn, Mariola Marx, Olaf Matuschek,
Dirk Riemann, Melanie Schuba, Leo Stoeckl, Katrin Tomanek, Stefan Waselikowski, and Geordie Williamson. 

I thank my family for their love and constant support.

This thesis is dedicated to the memory of my Grandmother, Joan Enright. Every Friday for the last three years of my high school career, I would stay the night with her, and play tennis the following morning. In the evening she would attempt, each time in vain, to teach me the rudiments of  Contract bridge, along with my friend Mark Respinger and her friend Anne Kelly. If every instance of failure were filled with such happy memories, no one could ever wish to succeed.}

\end{chapter}
